Recovering Plasticity of Neural Networks via Soft Weight Rescaling

Recent studies have shown that as training progresses, neural networks gradually lose their capacity to learn new information, a phenomenon known as plasticity loss. An unbounded weight growth is one of the main causes of plasticity loss. Furthermore, it harms generalization capability and disrupts optimization dynamics. Re-initializing the network can be a solution, but it results in the loss of learned information, leading to performance drops. In this paper, we propose Soft Weight Rescaling (SWR), a novel approach that prevents unbounded weight growth without losing information. SWR recovers the plasticity of the network by simply scaling down the weight at each step of the learning process. We theoretically prove that SWR bounds weight magnitude and balances weight magnitude between layers. Our experiment shows that SWR improves performance on warm-start learning, continual learning, and single-task learning setups on standard image classification benchmarks.

==> figures/initialization.tex <==


\begin{figure}[!h]
\centering
    \centering\captionsetup{width=.95\linewidth}%
    \includegraphics[width=\linewidth]{figures/sources/dummy_limited_bn.png}
    \caption{
    \textbf{Results across different initialization techniques.} 
    The test accuracy with training 10 chunks. 
    For each chunk, the model is trained for 100 epochs and it cannot be accessed when training the next chunk. 
    \textcolor{red}{The left or (a) denotes bla bla bla, and the right or (b) represents bla bla blas.}
    }
    \label{fig:initialization}
\end{figure}



==> tables/hyperparameter_limited.tex <==


\begin{table}[ht]
    
    \centering
    \resizebox{0.6\columnwidth}{!}{%
        \begin{tabular}{l|l|c}
        Dataset & Method & Hyperparameter Set \\
        \hline
                     & S\&P & $\lambda=0.4$ \\
        MNIST        & L2      & $\lambda=1\mathrm{e}{-5}$ \\
        (MLP)        & L2 Init & $\lambda=1\mathrm{e}{-5}$ \\
                      & SWR    & $ \lambda=1\mathrm{e}{-4}$ \\
        \hline
                     & S\&P & $\lambda=0.8$ \\
        CIFAR-10     & L2      & $\lambda=1\mathrm{e}{-2}$ \\
        (CNN)        & L2 Init & $\lambda=1\mathrm{e}{-2}$ \\
                     & SWR     & $ \lambda=1\mathrm{e}{-3}$ \\
        \hline
                     & S\&P & $\lambda=0.8$ \\
        CIFAR-100     & L2      & $\lambda=1\mathrm{e}{-2}$ \\
        (CNN)        & L2 Init & $\lambda=1\mathrm{e}{-2}$ \\
                     & SWR     & $ \lambda=1\mathrm{e}{-3}$ \\
        \hline
                     & S\&P & $\lambda=0.8$ \\
        CIFAR100     & L2      & $ \lambda=1\mathrm{e}{-2}$ \\
        (CNN-BN)     & L2 Init & $\lambda =1\mathrm{e}{-2}$ \\
                     & SWR     & $\lambda_f=1\mathrm{e}{-4}, \lambda_c=1\mathrm{e}{+0}$ \\
        \hline
                     & S\&P & $\lambda=0.8$ \\
        TinyImageNet & L2      & $\lambda=1\mathrm{e}{-5}$ \\
        (VGG16-BN)   & L2 Init & $\lambda=1\mathrm{e}{-5}$ \\
                     & SWR     & $\lambda_f=1\mathrm{e}{-2}, \lambda_c=1\mathrm{e}{-1}$ \\
        \end{tabular}%
    }
    \caption{Hyperparameter set of each method on continual limited access experiment.} 
    \label{tab:hyperparameter_limited}
\end{table}


